A Multi-criteria Approach to Evolve Sparse Neural Architectures for Stock Market Forecasting

This study proposes a new framework to evolve efficacious yet parsimonious neural architectures for the movement prediction of stock market indices using technical indicators as inputs. In the light of a sparse signal-to-noise ratio under the Efficient Market hypothesis, developing machine learning methods to predict the movement of a financial market using technical indicators has shown to be a challenging problem. To this end, the neural architecture search is posed as a multi-criteria optimization problem to balance the efficacy with the complexity of architectures. In addition, the implications of different dominant trading tendencies which may be present in the pre-COVID and within-COVID time periods are investigated. An $\epsilon-$ constraint framework is proposed as a remedy to extract any concordant information underlying the possibly conflicting pre-COVID data. Further, a new search paradigm, Two-Dimensional Swarms (2DS) is proposed for the multi-criteria neural architecture search, which explicitly integrates sparsity as an additional search dimension in particle swarms. A detailed comparative evaluation of the proposed approach is carried out by considering genetic algorithm and several combinations of empirical neural design rules with a filter-based feature selection method (mRMR) as baseline approaches. The results of this study convincingly demonstrate that the proposed approach can evolve parsimonious networks with better generalization capabilities.

==> Raw__Literature_review.tex <==
(XYZ this file contains the raw snips of text for the literature review XYZ)
The quest for efficient forecasting algorithms for stock values and stock market indices  has  a long history \cite{Regnault1863,Bachelier1900}. One of the proven classical tools for financial times series forecasting is  Auto Regressive Integrated Moving Average model (ARIMA), combined with exponential smoothing and de-trending and de-seasonalizing.  The ARIMA algorithm forecasts the value of the time series by an optimally weighted sum of lagged values each with a corresponding error term. To expand on the information which can  support  the forecasting of the target time series, a non-linear auto regressive exogenous model  (NARX) can be applied,  in which an external driving time series which influences the target series is included. (TO BE EXPANDED)\\

The critique of Makridakis et al on ANN performance with respect to statistical time series techniques \cite{Makridakis2018} (TO BE EXPANDED)\\

The \emph{efficient market hypothesis} (EMH) questions the possibility to `beat the market', i.e. consistently predict the movement prior to the stock market's re-evaluation of the price. The EMH states that a current market price reflects all available information through an efficiently integrating process - see e.g. Fama's work \cite{Fama1965}. While this understanding of the impossibility to capitalize on available information to forecast future prices is supposed generally valid,  more recent studies have found occurrences of occasional or repetitive anomalies in this behavior, e.g. in the \emph{adaptive market hypothesis} approach by Urquhart \emph{et al.} \cite{Urquhart2013} or the \emph{inefficient market hypothesis} by Asadi \emph{et al.} \cite{Asadi2012}.
A classifier hence must learn the purportedly remaining \emph{signal} within the  dominant random evolution of the stock market times series resulting in lower accuracy thresholds.
Zhong and Enke \cite{Zhong2019} tested DNNs to predict the daily return direction of stock market indices based on 60 financial and economic features.  Their simulation results show that the DNNs using untransformed  datasets (of 60 indicators including several exogenous parameters) and up to 18 hidden layers  achieved and accuracy of up to 58.6\% in testing data. (TO BE EXPANDED)\\

Hewamalage et al refute Makridakis critique on the performance of ANN - RNN with respect to classical statistical time-series analysis \cite{Hewamalage2021}. (TO BE EXPANDED)\\

{\bf Literature Review -  ANN and stock movement prediction}

\cite{Kim2003}, Kim applies SVM (Support vector machine) to forecasting Financial time series direction by implementing a risk function of the empirical error and `regularized term' based on structural risk (and compares to SVM  to BPNN  and case-based reasoning). 
Classical NN models used  \emph{empirical risk minimization}  (miss classification) while SVM implements the \emph{structural risk} (setting upper bound on the generalization error).  
% 
Uses 12 Technical Indicators in the SVM {\bf classifier} on the data set Korea composite stock price index (KOSPI).: 2928 trading days, from January 1989 to December 1998. 
%About 20\% of the data is used for holdout and 80\% for training. The number of the training data is 2347 and that of the holdout data is 581. The holdout data is used to test results with the data that is not utilized to develop the model. 
%The measure of prediction performance P is average of  (TP + TN / all ) hence accuracy.
% Structure of BPNN 1 hidden layer with 6, 12 or 24 hidden nodes   where sigmoid is used, while PureLin function on the output. 
Best SVM results in performance on holdout 57.8313 \% (depending on the kernel parameter of Gaussian radial basis function  plane and the boundary on the coefficients of the separation hyper plane), while 54.7332 \% for BPNN.\\
\cite{Huang2009};  Huang and Tsai  implement filter-based feature selection, self-organizing feature map (SOFM) out of 13 TI,  to cluster the training samples (and to reduce training time) and SVR  (SVM {\bf regressor}) to forecast the stock market price index. The  data set is  the Taiwan index futures (FITX) to predict the next day’s {\bf price index} with 5 year+3 months training and almost 3 tailing months of test data. Implementation of one SVR for each cluster (3,4 or 5) of data samples results in  average MAPE errors respectively  3.59002\%, 3.90044\%, and 4.3148\%.\\
\cite{Kara2011}; Kara, Boyacioglu and Baykan implement  ANN and SVM with ten technical indicators as features to forecast  the stock price  index direction of movement. The data set is daily Istanbul Stock Exchange (ISE) National 100 Index. The models are based on two classification techniques, ANN and SVM.  Two comprehensive parameter settings show performance of the ANN model at 75.74\% outperforming  SVM model  at 71.52\%. (XYZ EXTREMELY HIGH VALUES requires explanation viz. the way this study constructs the \emph{train} set to mimic the \emph{test} set  XYZ )
Period from January 2, 1997 to December 31, 2007. 
%The total number of cases is 2733 trading days. The number of cases with increasing direction is 1440 while the number of cases with decreasing direction is 1293. 
for which  52.7\% of  all cases have an increasing direction.% and 47.3% of the all cases have a decreasing direction. 
 The parameter setting training (set is of size 20\%) is taken \emph{`proportional to the number of increases and decreases for each year in the entire data set'. }
Ten TI were used, 1 hidden layer to minimize RMS\%, with  tanh on the hidden layer and the logistic sigmoid activation on the output layer. 
The number of neurons (n, 10 to 100) in the hidden layer, value of learning rate (lr =.1), momentum constant (mc, .1 to .9) and number of iterations (ep, 1000 to 10000) in the ANN were tested. The best prediction accuracy  on holdout  data 82.48 (Lr = .1ep = 5000, mc.7,  n = 30) worst 68.29 (year 2003, 7000,.1,90). In this study SVM underperforms relative to BPNN.\\
\cite{Asadi2012}: Asadi, Hadavandi, Mehmanpazir and Nakhostin implement a combination of data preprocessing methods, genetic algorithms (GA) and the Levenberg–Marquardt (LM) algorithm - `damped' gradient interpolating Gauss-Newton algorithm and Gradient Descent -  in   PELMNN (pre-processed evolutionary LM neural networks). The authors point out the advantage of  GA to not require a differentiable error function and  provide flexibility of  fitness expression  to include additional  criteria.   Using four stages i) data pre-processing by scaling and stepwise regression analysis (SRA) to select    key variables, ii)   genetic algorithm to evolve  initial weights in the Evolutionary Neural Network, iii) tune  weights  of the ENN using LMBP and iv) post-process (return to scale) the outcomes for forecasting .
Study gives  performance by mean absolute percentage error (MAPE) , prediction of change in direction (POCID),  the Theil statistic  which compares to random prediction ( `future prediction is present value') and finally the  Average Relative Variance (ARV) which compares to mean value prediction.\\
Their  study takes 7 TI and 620  data   points  with 500 to train and final 120 points as test data - in a window that was chosen differently for each of seven stock market indices TSE, TEPIX, DJIA and NASDAQ (not reported about 50 Companies Index, Industry Index and Financial Group Index ).
The models delivers results of POCID values 57.5 (Index of Top 50 Companies )  to   94.16 (NASDAQ). (XYZ extremely high value for the NASDAQ  - why ? XYZ)\\
\cite{Chang2012}: Chang, Wang and Zhou develop evolving partially connected neural networks (EPCNN which  consists in  (1) provide number of neurons and layers; (2) normalize input variables; (3) initialize weights and make sure that the neurons are connected; (4) calculate the output value by inputting variables into the network; (5) search optimal or near-optimal connection weights by GA; (6) store optimized weights.  The features are 24 TI, the  activation function is $ \sin(x)$ function, the data set is S\&P500 for the window  training samples from January 2008 to December 2008  and testing samples form January 2009 to June 2009. \\
The selected stocks are Citigroup and Motors Liquidation Company. The historic data is collected form S\&P 500 and covers the financial time-series data from 2008/01/01 to 2009/6/31. The historic data from 2008/ 01/01 to 2008/12/31 is used for training and the historic data from 2009/01/01 to 2009/06/31 is used for testing. For Citigroup, the size of the training and test data is 254 and 124, respectively. For Motors Liquidation Company the size of the training and test data respectively is 253 and 124. The percentage accuracy is defined as   $\vert  \widehat y_t - y_t \vert  < \alpha$ then prediction is successful. The $\alpha$ in \emph{test} was taken at a value of 1 (for Citigroup) and results in an accuracy of e.g.   97.58 \% (Citigroup) when the EPCNN is initially configured at 50 neurons in 4 layers.\\
% MAPE for TSE of .501
\cite{Wu2014}; Wu, Yu and Chang develop an intelligent stock trading system using comprehensive features (ISTSCF) , and generated by {\bf sentiment analysis} (SA) on sensitive market events from stock news articles.  The model uses SVR  with inputs of text  (nominal stock messages) and TI, implements trend-based  segmentation method. Predict `buy' and `sell'  or `hold' signal based on thresholds. Efficiency assessment by \emph{trade profit rate} on the Taiwan stock market shows TI(SRA)+SI outperforms classical TI approaches (stepwise regression analysis, SRA).\\
\cite{Nayak2015}; Nayak,  Mishra and Rath combine  SVM to classify stock data and KNN  to predict  closing price, volatility and momentum of the stock market. Uses 8 TI on a dataset from BSE-SENSEX and CNX Nifty ( last 700 samples prior to August 2104 were taken out of which 500 for training and last 200 samples are used for testing. ). For the 1-day forecasting of the former index their SVM-KNN obtains an MAPE of 0.06 in comparison to models FLIT2FNS at .23  and CEFLANN at .56 .
 
\cite{kumar:Meghwani:2016}; Kumar, Meghwani and  Thakur  propose a model which uses a feature selection procedure  and  a proximal support vector machine to forecast one-day-ahead the direction of stock indices. Four feature selection procedure are compared Linear Correlation, Rank Correlation, Regression Relief and Random Forest, and 55 TI  are used on twelve market indices. Results show the best performance of RF-PSVM. Data window  January 2008 to December 2013, with training from January 2008 to December 2012 and testing from January 2013 to December 2013. 
 
\cite{Ye2016};
% A novel forecasting method based on multi-order fuzzy time series and technical analysis.
% Furong Ye, Liming Zhang, Defu Zhang, Hamido Fujita , Zhiguo Gong 
Ye et al. build a multi-order  - exponentially smoothed - \emph{fuzzy} time series (from technical indicators like ROC, MACD and KDJ) analysis which optimizes  RMSE, MSE and  DAR (Directional Accuracy Rate) and forecasts closing values for five stock market indices. In this approach fuzzy logical relationships are extracted from the fuzzified training data of January-October, of which the domain has been optimally segmented by use of a genetic algorithm, and are tested in fuzzified data of November-December. The study reports results of DAR around or higher than 60 \% for the different stock-indexes (NASDAQ DAR-average 1999-2004 at 68.39\%).

\cite{Weng2017}; Weng and Fadel use ``crowd-sourced'' knowledge bases in addition to technical indicators. The Efficient Market Hypothesis states that stock prices are reacting to information and can therefor not be predicted from historic values or derived technical indicators.
Using external features from daily counts of Google News related to a given stock and the number of unique visitors to pertinent Wikipedia pages and three TI (Stochastic Oscillator, Larry Williams momentum indicator, Relative Strength Index), their study reports an 85\% accuracy in predicting the next-day AAPL stock movement (with SVM and DT classifiers).

\cite{Lei2018}; Lei proposes a model in which first the Rough Set (RS) approach is used to reduce the number of feature dimensions for forecasting stock market index trend (5 cases) and to reduce number of nodes in the hidden layers of the  Wavelet Neural Network (WNN). In the WNN model each output is a linear combination of  wavelet function values of the one hidden layer nodes. The model selects from fifteen technical indicators and obtains Directional Symmetry values of about 66 \%.
(data for training and testing compare 500/100 but no absolute time window reported)

\cite{Xu2018}
% Stock Movement Prediction from Tweets and Historical Prices. Yumo Xu and Shay B. Cohen
Xu and Cohen apply NLP analysis of social media corpora (Twitter querying for Nasdaq ticker symbols) and a Variational Movement Decoder (with forward and backward GRU) and temporal attention in their StockNet model. 
The data sets consist of 88 stocks from January 2014 till January 2016, removing stocks in the 50-55\% movement direction range: 20339 movements for training and 3720 movements for testing.
Performance evaluated by classification accuracy and Matthews Correlation Coefficient.
The StockNet model improves over the HAN model by acc = 58.23 and MCC = 0.081.

\cite{Dash2019}; Dash et al use an MCDM approach - Technique for Order Preference by Similarity to Ideal Solution (TOPSIS) - for selecting and ranking among seven classifiers RBFN, MLP, SVM,KNN,DT, LR and NB, and Crow Search for weighting. The study  uses seven performance measures TP, TN, Acc, F1, Precision, Recall and G-mean, six technical indicators over 685 samples (70/30 for train/test),  1st January 2015 - 13 th November 2017, for each of three indices BSE SENSEX, SP500 and NIFTY50. On average acc of .85 are reported for the best performer TOPSIS-CS-WV (Weighted Voting).

\cite{Hoseinzade2019}; Hoseinzade and Haratizadeh apply convolutional neural network (CNN) to forecast next-day direction of movement of markets (SP500, NASDAQ, DJIA, NYSE, RUSSEL) using various sources besides the market based indicators; exchange rate of currencies, future contracts, price of commodities, other global market indices, price of major US companies and treasury bill rates (82 in total).
Uses a 3-dimensional tensor (past days $\times$ markets $\times$ features) to aggregate all input data and subsequently extracts relevant features for prediction by filter. Data window is Jan 2010 to Nov 2017 split in 60\% training, 20 \% validation and 20 \% testing. Performance measured by macro-averaged F-measure (mean of F measure for both classes) - selection of best algorithms average  0.56 for the different markets. 
% 0.5532 0.5612 0.5576 0.5592 0.5787

\cite{Tang2019}; Tang, Dong and Shi focus on turning points (TPs) or time point safter which longer periods of fall or rise occur and hence aim to implement piecewise linear representations at instances forecasted by weighted SVM (WSVM).
 The used  data set holds 20 random stocks from Shanghai Stock Exchange (4th Jan 2010 to 18 th Aug 2011), for which the model provides trading signals using RSI (Relative Strength Index to signal buying or selling) and DODS (delay one day strategy). Model performance measured by average revenue or coefficient of variation.
 
%\cite{Kia2020} Network-based direction of movement prediction in financial markets. % Arash Negahdari Kia, Saman Haratizadeh, Saeed Bagheri Shouraki
%The model of Kia, Haratizadeh and Shouraki uses semi-supervised graph-based to prediction market direction of movement.

\cite{UlHaq2021}; The work of Haq et al starts with forty-four technical indicators for  eighty-eight stocks to compute their importance by independently training logistic regression model, support vector machine and random forests. The most relevant features are further input into  a deep generative model with a market signal extractor (market movement) and an attention mechanism (predictive dependencies of different temporal auxiliary outputs). The data set is the same as the one used in \cite{Xu2018} and shows StockNet  combined with multi-filter feature selection (MFFS) achieves   59.44\% accuracy and 0.1030 MCC.

